Field study on requirements engineering: Investigation of artefacts, project parameters, and execution strategies

Requirements Engineering (RE) is a critical discipline mostly driven by uncertainty, since it is influenced by the customer domain or by the development process model used. We aim to investigate RE processes in successful project environments to discover characteristics and strategies that allow us to elaborate RE tailoring approaches in the future. We perform a field study on a set of projects at one company. First, we investigate by content analysis which RE artefacts were produced in each project and to what extent they were produced. Second, we perform qualitative analysis of semi-structured interviews to discover project parameters that relate to the produced artefacts. Third, we use cluster analysis to infer artefact patterns and probable RE execution strategies, which are the responses to specific project parameters. Fourth, we investigate by statistical tests the effort spent in each strategy in relation to the effort spent in change requests to evaluate the efficiency of execution strategies. Our results show no statistically significant difference between the efficiency of the strategies. In addition, it turned out that many parameters considered as the main causes for project failures can be successfully handled. Hence, practitioners can apply the artefact patterns and related project parameters to tailor the RE process according to individual project characteristics.

==> 2011 IST Journal/projectparametertable.tex <==
~

 &  
\multicolumn{1}{c||}{
~
}
 &  
\multicolumn{10}{c||}{
Business Needs Artefacts~
}
 &  
 
 
 
 
 
 
 
 
 
\multicolumn{13}{c||}{
Requirements Specification Artefacts~
}
 &  
 
 
 
 
 
 
 
 
 
 
 
 
\multicolumn{14}{c||}{
System Specification Artefacts~
}
 &  
 
 
 
 
 
 
 
 
 
 
 
 
 
\multicolumn{2}{c||}{
Traceability~
}
 
 \\ \cline{3-41} 
\multicolumn{1}{||c||}{
~
}
 &  
\multicolumn{1}{c||}{
~
}
 &  
\multicolumn{10}{c||}{
~
}
 &  
 
 
 
 
 
 
 
 
 
\multicolumn{4}{c||}{
Functional~
}
 &  
 
 
 
\multicolumn{9}{c||}{
Non-functional~
}
 &  
 
 
 
 
 
 
 
 
\multicolumn{11}{c||}{
Design Concept~
}
 &  
 
 
 
 
 
 
 
 
 
 
\multicolumn{3}{c||}{
Test~
}
 &  
 
 
\multicolumn{2}{c||}{
~
}
 
 \\ \hline\hline 
Category~
 &  
Project Parameter~
 &  
\begin{sideways}Business Objectives~\end{sideways}
 &  
\begin{sideways}Customer Requirements~\end{sideways}
 &  
\begin{sideways}Value to Customer~\end{sideways}
 &  
\begin{sideways}Main Features~\end{sideways}
 &  
\begin{sideways}Assumptions and Dependcies~\end{sideways}
 &  
\begin{sideways}Scope and Limitations~\end{sideways}
 &  
\begin{sideways}ROI Calculations~\end{sideways}
 &  
\begin{sideways}Business Risk Analysis~\end{sideways}
 &  
\begin{sideways}Risk Calculations~\end{sideways}
 &  
\begin{sideways}System Success Factors~\end{sideways}
 &  
\begin{sideways}Application Scenarios~\end{sideways}
 &  
\begin{sideways}User Interface~\end{sideways}
 &  
\begin{sideways}User Classes~\end{sideways}
 &  
\begin{sideways}System Interaction~\end{sideways}
 &  
\begin{sideways}Release Strategy~\end{sideways}
 &  
\begin{sideways}Domain Model~\end{sideways}
 &  
\begin{sideways}Environment Model~\end{sideways}
 &  
\begin{sideways}System Boundaries~\end{sideways}
 &  
\begin{sideways}Quality Requirements~\end{sideways}
 &  
\begin{sideways}Assumptions~\end{sideways}
 &  
\begin{sideways}SW Design Constraints~\end{sideways}
 &  
\begin{sideways}Acceptance Criteria~\end{sideways}
 &  
\begin{sideways}Acceptance Test Cases~\end{sideways}
 &  
\begin{sideways}Release Planning~\end{sideways}
 &  
\begin{sideways}Behaviour Model~\end{sideways}
 &  
\begin{sideways}System Interaction~\end{sideways}
 &  
\begin{sideways}Service Interaction~\end{sideways}
 &  
\begin{sideways}Data Model~\end{sideways}
 &  
\begin{sideways}User Interface~\end{sideways}
 &  
\begin{sideways}Communication Interfaces~\end{sideways}
 &  
\begin{sideways}Interfaces to Service Comp.~\end{sideways}
 &  
\begin{sideways}Architecture Constraints~\end{sideways}
 &  
\begin{sideways}Deployment Constraints~\end{sideways}
 &  
\begin{sideways}Coding Standards~\end{sideways}
 &  
\begin{sideways}Functional Test Criteria~\end{sideways}
 &  
\begin{sideways}Integration Test Criteria~\end{sideways}
 &  
\begin{sideways}Design Constr. Test Criteria~\end{sideways}
 &  
\begin{sideways}Needs to Requirements~\end{sideways}
 &  
\begin{sideways}Requirements to Sys.Spec~\end{sideways}
 \\ \hline\hline 
\multirow{8}{*}{
\begin{sideways}Customers' Domain~\end{sideways}
}
 &  
Governmental customer~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 \\ \cline{2-41} 
\multirow{8}{*}{
\begin{sideways}~\end{sideways}
}
 &  
Weak access to business processes~
 &  
~
 &  
~
 &  
-~
 &  
~
 &  
+~
 &  
~
 &  
-~
 &  
-~
 &  
+~
 &  
~
 &  
-~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
-~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
-~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
-~
 &  
~
 &  
~
 &  
~
 &  
~
 \\ \cline{2-41} 
\multirow{8}{*}{
\begin{sideways}~\end{sideways}
}
 &  
Weak relation to customer ~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
+~
 &  
+~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
+~
 \\ \cline{2-41} 
\multirow{8}{*}{
\begin{sideways}~\end{sideways}
}
 &  
Good relation to customer~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
-~
 &  
~
 &  
~
 &  
~
 &  
-~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 \\ \cline{2-41} 
\multirow{8}{*}{
\begin{sideways}~\end{sideways}
}
 &  
Weak knowledge on customer's domain~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 \\ \cline{2-41} 
\multirow{8}{*}{
\begin{sideways}~\end{sideways}
}
 &  
Unavailability of stakeholders~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
+~
 &  
-~
 &  
-~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
-~
 &  
~
 &  
-~
 &  
+~
 &  
~
 &  
+~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 \\ \cline{2-41} 
\multirow{8}{*}{
\begin{sideways}~\end{sideways}
}
 &  
Weak technical ability of stakeholders ~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
-~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 \\ \cline{2-41} 
\multirow{8}{*}{
\begin{sideways}~\end{sideways}
}
 &  
Unreliability of stakeholders ~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
-~
 &  
~
 &  
~
 &  
+~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 \\ \hline\hline 
\multirow{10}{*}{
\begin{sideways}\centering\begin{minipage}{3cm}\centering System under \\Consideration\end{minipage}~\end{sideways}
}
 &  
High degree of user interaction~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
+~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
+~
 &  
+~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 \\ \cline{2-41} 
\multirow{10}{*}{
\begin{sideways}~\end{sideways}
}
 &  
High degree of innovation ~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
+~
 &  
~
 &  
+~
 &  
+~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 \\ \cline{2-41} 
\multirow{10}{*}{
\begin{sideways}~\end{sideways}
}
 &  
Emphasise on data flow ~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
-~
 &  
-~
 &  
-~
 &  
-~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
+~
 &  
-~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 \\ \cline{2-41} 
\multirow{10}{*}{
\begin{sideways}~\end{sideways}
}
 &  
Emphasise on control flow ~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
+~
 &  
+~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
+~
 &  
~
 &  
+~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 \\ \cline{2-41} 
\multirow{10}{*}{
\begin{sideways}~\end{sideways}
}
 &  
High degree of distribution~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
+~
 &  
+~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
+~
 &  
+~
 &  
-~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 \\ \cline{2-41} 
\multirow{10}{*}{
\begin{sideways}~\end{sideways}
}
 &  
Complex dependencies to external systems~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
-~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 \\ \cline{2-41} 
\multirow{10}{*}{
\begin{sideways}~\end{sideways}
}
 &  
Weak knowledge on operative environment~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
-~
 &  
-~
 &  
-~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
-~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
-~
 &  
~
 &  
~
 &  
~
 \\ \cline{2-41} 
\multirow{10}{*}{
\begin{sideways}~\end{sideways}
}
 &  
Weak knowledge on op. background ~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
-~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
-~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 \\ \cline{2-41} 
\multirow{10}{*}{
\begin{sideways}~\end{sideways}
}
 &  
Custom software~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 \\ \cline{2-41} 
\multirow{10}{*}{
\begin{sideways}~\end{sideways}
}
 &  
Standard software~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
-~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
-~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 \\ \hline\hline 
\multirow{13}{*}{
\begin{sideways}Cross-Cutting Process Aspects~\end{sideways}
}
 &  
Time-boxing~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
+~
 \\ \cline{2-41} 
\multirow{13}{*}{
\begin{sideways}~\end{sideways}
}
 &  
Existence external parties~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 \\ \cline{2-41} 
\multirow{13}{*}{
\begin{sideways}~\end{sideways}
}
 &  
External acceptance tests~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
+~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
+~
 \\ \cline{2-41} 
\multirow{13}{*}{
\begin{sideways}~\end{sideways}
}
 &  
Explicit assignment of RE~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 \\ \cline{2-41} 
\multirow{13}{*}{
\begin{sideways}~\end{sideways}
}
 &  
High amount of requirements~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
+~
 \\ \cline{2-41} 
\multirow{13}{*}{
\begin{sideways}~\end{sideways}
}
 &  
Long project duration~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
+~
 \\ \cline{2-41} 
\multirow{13}{*}{
\begin{sideways}~\end{sideways}
}
 &  
Estimations of functional complexity~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 \\ \cline{2-41} 
\multirow{13}{*}{
\begin{sideways}~\end{sideways}
}
 &  
Weak given documentation~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 \\ \cline{2-41} 
\multirow{13}{*}{
\begin{sideways}~\end{sideways}
}
 &  
Change mgmt. established~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
+~
 \\ \cline{2-41} 
\multirow{13}{*}{
\begin{sideways}~\end{sideways}
}
 &  
Standardised design process~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
+~
 &  
+~
 &  
+~
 &  
+~
 &  
+~
 &  
+~
 &  
+~
 &  
+~
 &  
+~
 &  
+~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 \\ \cline{2-41} 
\multirow{13}{*}{
\begin{sideways}~\end{sideways}
}
 &  
High team-size~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 \\ \cline{2-41} 
\multirow{13}{*}{
\begin{sideways}~\end{sideways}
}
 &  
High team distribution~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 \\ \cline{2-41} 
\multirow{13}{*}{
\begin{sideways}~\end{sideways}
}
 &  
Weak experience team~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
-~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 \\ \hline\hline 


==> projectparametertable.tex <==
~

 &  
\multicolumn{1}{c||}{
~
}
 &  
\multicolumn{10}{c||}{
Business Needs Artefacts~
}
 &  
 
 
 
 
 
 
 
 
 
\multicolumn{13}{c||}{
Requirements Specification Artefacts~
}
 &  
 
 
 
 
 
 
 
 
 
 
 
 
\multicolumn{14}{c||}{
System Specification Artefacts~
}
 &  
 
 
 
 
 
 
 
 
 
 
 
 
 
\multicolumn{2}{c||}{
Traceability~
}
 
 \\ \cline{3-41} 
\multicolumn{1}{||c||}{
~
}
 &  
\multicolumn{1}{c||}{
~
}
 &  
\multicolumn{10}{c||}{
~
}
 &  
 
 
 
 
 
 
 
 
 
\multicolumn{4}{c||}{
Functional~
}
 &  
 
 
 
\multicolumn{9}{c||}{
Non-functional~
}
 &  
 
 
 
 
 
 
 
 
\multicolumn{11}{c||}{
Design Concept~
}
 &  
 
 
 
 
 
 
 
 
 
 
\multicolumn{3}{c||}{
Test~
}
 &  
 
 
\multicolumn{2}{c||}{
~
}
 
 \\ \hline\hline 
Category~
 &  
Project Parameter~
 &  
\begin{sideways}Business Objectives~\end{sideways}
 &  
\begin{sideways}Customer Requirements~\end{sideways}
 &  
\begin{sideways}Value to Customer~\end{sideways}
 &  
\begin{sideways}Main Features~\end{sideways}
 &  
\begin{sideways}Assumptions and Dependcies~\end{sideways}
 &  
\begin{sideways}Scope and Limitations~\end{sideways}
 &  
\begin{sideways}ROI Calculations~\end{sideways}
 &  
\begin{sideways}Business Risk Analysis~\end{sideways}
 &  
\begin{sideways}Risk Calculations~\end{sideways}
 &  
\begin{sideways}System Success Factors~\end{sideways}
 &  
\begin{sideways}Application Scenarios~\end{sideways}
 &  
\begin{sideways}User Interface~\end{sideways}
 &  
\begin{sideways}User Classes~\end{sideways}
 &  
\begin{sideways}System Interaction~\end{sideways}
 &  
\begin{sideways}Release Strategy~\end{sideways}
 &  
\begin{sideways}Domain Model~\end{sideways}
 &  
\begin{sideways}Environment Model~\end{sideways}
 &  
\begin{sideways}System Boundaries~\end{sideways}
 &  
\begin{sideways}Quality Requirements~\end{sideways}
 &  
\begin{sideways}Assumptions~\end{sideways}
 &  
\begin{sideways}SW Design Constraints~\end{sideways}
 &  
\begin{sideways}Acceptance Criteria~\end{sideways}
 &  
\begin{sideways}Acceptance Test Cases~\end{sideways}
 &  
\begin{sideways}Release Planning~\end{sideways}
 &  
\begin{sideways}Behaviour Model~\end{sideways}
 &  
\begin{sideways}System Interaction~\end{sideways}
 &  
\begin{sideways}Service Interaction~\end{sideways}
 &  
\begin{sideways}Data Model~\end{sideways}
 &  
\begin{sideways}User Interface~\end{sideways}
 &  
\begin{sideways}Communication Interfaces~\end{sideways}
 &  
\begin{sideways}Interfaces to Service Comp.~\end{sideways}
 &  
\begin{sideways}Architecture Constraints~\end{sideways}
 &  
\begin{sideways}Deployment Constraints~\end{sideways}
 &  
\begin{sideways}Coding Standards~\end{sideways}
 &  
\begin{sideways}Functional Test Criteria~\end{sideways}
 &  
\begin{sideways}Integration Test Criteria~\end{sideways}
 &  
\begin{sideways}Design Constr. Test Criteria~\end{sideways}
 &  
\begin{sideways}Needs to Requirements~\end{sideways}
 &  
\begin{sideways}Requirements to Sys.Spec~\end{sideways}
 \\ \hline\hline 
\multirow{8}{*}{
\begin{sideways}Customers' Domain~\end{sideways}
}
 &  
Governmental customer~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 \\ \cline{2-41} 
\multirow{8}{*}{
\begin{sideways}~\end{sideways}
}
 &  
Weak access to business processes~
 &  
~
 &  
~
 &  
-~
 &  
~
 &  
+~
 &  
~
 &  
-~
 &  
-~
 &  
+~
 &  
~
 &  
-~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
-~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
-~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
-~
 &  
~
 &  
~
 &  
~
 &  
~
 \\ \cline{2-41} 
\multirow{8}{*}{
\begin{sideways}~\end{sideways}
}
 &  
Weak relation to customer ~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
+~
 &  
+~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
+~
 \\ \cline{2-41} 
\multirow{8}{*}{
\begin{sideways}~\end{sideways}
}
 &  
Good relation to customer~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
-~
 &  
~
 &  
~
 &  
~
 &  
-~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 \\ \cline{2-41} 
\multirow{8}{*}{
\begin{sideways}~\end{sideways}
}
 &  
Weak knowledge on customer's domain~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 \\ \cline{2-41} 
\multirow{8}{*}{
\begin{sideways}~\end{sideways}
}
 &  
Unavailability of stakeholders~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
+~
 &  
-~
 &  
-~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
-~
 &  
~
 &  
-~
 &  
+~
 &  
~
 &  
+~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 \\ \cline{2-41} 
\multirow{8}{*}{
\begin{sideways}~\end{sideways}
}
 &  
Weak technical ability of stakeholders ~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
-~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 \\ \cline{2-41} 
\multirow{8}{*}{
\begin{sideways}~\end{sideways}
}
 &  
Unreliability of stakeholders ~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
-~
 &  
~
 &  
~
 &  
+~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 \\ \hline\hline 
\multirow{10}{*}{
\begin{sideways}\centering\begin{minipage}{3cm}\centering System under \\Consideration\end{minipage}~\end{sideways}
}
 &  
High degree of user interaction~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
+~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
+~
 &  
+~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 \\ \cline{2-41} 
\multirow{10}{*}{
\begin{sideways}~\end{sideways}
}
 &  
High degree of innovation ~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
+~
 &  
~
 &  
+~
 &  
+~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 \\ \cline{2-41} 
\multirow{10}{*}{
\begin{sideways}~\end{sideways}
}
 &  
Emphasise on data flow ~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
-~
 &  
-~
 &  
-~
 &  
-~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
+~
 &  
-~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 \\ \cline{2-41} 
\multirow{10}{*}{
\begin{sideways}~\end{sideways}
}
 &  
Emphasise on control flow ~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
+~
 &  
+~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
+~
 &  
~
 &  
+~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 \\ \cline{2-41} 
\multirow{10}{*}{
\begin{sideways}~\end{sideways}
}
 &  
High degree of distribution~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
+~
 &  
+~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
+~
 &  
+~
 &  
-~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 \\ \cline{2-41} 
\multirow{10}{*}{
\begin{sideways}~\end{sideways}
}
 &  
Complex dependencies to external systems~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
-~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 \\ \cline{2-41} 
\multirow{10}{*}{
\begin{sideways}~\end{sideways}
}
 &  
Weak knowledge on operative environment~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
-~
 &  
-~
 &  
-~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
-~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
-~
 &  
~
 &  
~
 &  
~
 \\ \cline{2-41} 
\multirow{10}{*}{
\begin{sideways}~\end{sideways}
}
 &  
Weak knowledge on op. background ~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
-~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
-~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 \\ \cline{2-41} 
\multirow{10}{*}{
\begin{sideways}~\end{sideways}
}
 &  
Custom software~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 \\ \cline{2-41} 
\multirow{10}{*}{
\begin{sideways}~\end{sideways}
}
 &  
Standard software~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
-~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
-~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 \\ \hline\hline 
\multirow{13}{*}{
\begin{sideways}Cross-Cutting Process Aspects~\end{sideways}
}
 &  
Time-boxing~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
+~
 \\ \cline{2-41} 
\multirow{13}{*}{
\begin{sideways}~\end{sideways}
}
 &  
Existence external parties~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 \\ \cline{2-41} 
\multirow{13}{*}{
\begin{sideways}~\end{sideways}
}
 &  
External acceptance tests~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
+~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
+~
 \\ \cline{2-41} 
\multirow{13}{*}{
\begin{sideways}~\end{sideways}
}
 &  
Explicit assignment of RE~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 \\ \cline{2-41} 
\multirow{13}{*}{
\begin{sideways}~\end{sideways}
}
 &  
High amount of requirements~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
+~
 \\ \cline{2-41} 
\multirow{13}{*}{
\begin{sideways}~\end{sideways}
}
 &  
Long project duration~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
+~
 \\ \cline{2-41} 
\multirow{13}{*}{
\begin{sideways}~\end{sideways}
}
 &  
Estimations of functional complexity~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 \\ \cline{2-41} 
\multirow{13}{*}{
\begin{sideways}~\end{sideways}
}
 &  
Weak given documentation~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 \\ \cline{2-41} 
\multirow{13}{*}{
\begin{sideways}~\end{sideways}
}
 &  
Change mgmt. established~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
+~
 \\ \cline{2-41} 
\multirow{13}{*}{
\begin{sideways}~\end{sideways}
}
 &  
Standardised design process~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
+~
 &  
+~
 &  
+~
 &  
+~
 &  
+~
 &  
+~
 &  
+~
 &  
+~
 &  
+~
 &  
+~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 \\ \cline{2-41} 
\multirow{13}{*}{
\begin{sideways}~\end{sideways}
}
 &  
High team-size~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 \\ \cline{2-41} 
\multirow{13}{*}{
\begin{sideways}~\end{sideways}
}
 &  
High team distribution~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 \\ \cline{2-41} 
\multirow{13}{*}{
\begin{sideways}~\end{sideways}
}
 &  
Weak experience team~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
+~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
-~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 &  
~
 \\ \hline\hline 

